Multi-Agent System for Orchestrating Retrieval and Multimodal Reasoning in Cloud Environments

Intelligent reasoning services in cloud environments increasingly support knowledge-intensive tasks such as multimodal generation and fact-checking. While large language models have greatly improved individual reasoning capability, existing systems often rely on single-agent designs and fixed inference pipelines, which are brittle under unreliable retrieval and partial execution failures. In this paper, we propose OR$^2$-MAS, a retrieval-augmented multi-agent framework designed to improve the robustness and efficiency of intelligent reasoning services through state-aware orchestration. OR$^2$-MAS coordinates retrieval and multi-agent reasoning through a global reasoning state, enabling adaptive routing, failure-aware redundancy, and dynamic control of reasoning depth. Experiments on multimodal fact-checking benchmarks show that OR$^2$-MAS achieves strong performance while remaining robust to retrieval and agent failures, highlighting the importance of system-level orchestration for cloud-based intelligent reasoning.

==> Tab/algorithm.tex <==
\begin{algorithm}[t]
\caption{OR$^2$-MAS: State-Aware Orchestration with Rule-Based Routing}
\label{alg:ormas}
\KwIn{User query $q$, initial hypothesis $\mathcal{H}_0$, agent pool $\mathcal{A}$, max rounds $T$, evidence budget $k$}
\KwOut{Final verdict $\hat{y}$, confidence $\hat{c}$, evidence $\mathcal{E}$}

$\mathcal{E}_0 \leftarrow \emptyset$\;
Initialize agent states $\mathcal{X}_0 = \{x_i^{(0)}=\texttt{pending}\}_{i\in\mathcal{A}}$\;

\For{$t=1$ \KwTo $T$}{
    \tcp{(1) Failure-aware redundancy (highest priority)}
    Compute failure ratio $\rho_t \leftarrow 
    \frac{1}{|\mathcal{A}_t|}\sum_{i\in\mathcal{A}_t}\mathbb{I}[x_i^{(t-1)}\in\{\texttt{timeout},\texttt{failure}\}]$\;
    \If{$\rho_t > \beta$}{
        $\mathcal{A}_t \leftarrow \textsc{Backup}(\mathcal{A}_t)$ \tcp*{spawn backup agents}
        $\mathcal{A}_t \leftarrow \textsc{Route}(\mathcal{A}_t)$  \tcp*{reroute pending subtasks}
    }

    \tcp{(2) Evidence acquisition (conservative OR trigger)}
    \If{$t=1$}{
        $\mathcal{E}_t \leftarrow \mathcal{E}_{t-1} \cup \textsc{Retrieve}(q,\mathcal{H}_{t-1},k)$\;
    }
    \Else{
        \If{$\mathcal{C}_{t-1} < \tau_c \ \vee\  \mathcal{U}_{t-1} > \tau_u$}{
            $\mathcal{E}_t \leftarrow \mathcal{E}_{t-1} \cup \textsc{Retrieve}(q,\mathcal{H}_{t-1},k)$\;
            $\texttt{no\_improve} \leftarrow \textsc{NotReduced}(\mathcal{U}_{t-1},\mathcal{U}_{t-2})$\;
            \If{$\texttt{no\_improve}$}{
                $\mathcal{A}_t \leftarrow \textsc{Route}(\mathcal{A}_t)$ \tcp*{diversify reasoning paths}
            }
        }
        \Else{
            $\mathcal{E}_t \leftarrow \mathcal{E}_{t-1}$\;
        }
    }

    \tcp{(3) Parallel multi-agent reasoning}
    \ForEach(\tcp*[f]{in parallel}){$a_i \in \mathcal{A}_t$}{
        $(y_i^{(t)}, c_i^{(t)}, h_i^{(t)}, x_i^{(t)}) \leftarrow 
        a_i(q,\mathcal{E}_t,\mathcal{H}_{t-1})$\;
    }

    \tcp{(4) Update global state: consensus and uncertainty}
    $\mathcal{C}_t \leftarrow \max_{\ell\in\mathcal{L}}
    \frac{1}{|\mathcal{A}_t^{ok}|}\sum_{i\in\mathcal{A}_t^{ok}}\mathbb{I}[y_i^{(t)}=\ell]$\;
    $\ell_t^\star \leftarrow \arg\max_{\ell\in\mathcal{L}}
    \sum_{i\in\mathcal{A}_t^{ok}}\mathbb{I}[y_i^{(t)}=\ell]$\;
    $\mathcal{U}_t \leftarrow 1-\frac{1}{|\mathcal{A}_t^{ok}|}
    \sum_{i\in\mathcal{A}_t^{ok}}\mathbb{I}[y_i^{(t)}=\ell_t^\star]\cdot c_i^{(t)}$\;
    $\mathcal{H}_t \leftarrow \textsc{RefineHypothesis}(q,\mathcal{E}_t,\{h_i^{(t)}\})$\;

    \tcp{(5) Adaptive termination}
    \If{$\mathcal{C}_t \ge \tau_c \ \wedge\  \mathcal{U}_t \le \tau_u$}{
        \textbf{break}\;
    }
}

\tcp{Aggregate final decision from last round}
$\hat{y} \leftarrow \ell_t^\star$\;
$\hat{c} \leftarrow \frac{1}{|\mathcal{A}_t^{ok}|}\sum_{i\in\mathcal{A}_t^{ok}}\mathbb{I}[y_i^{(t)}=\hat{y}]\cdot c_i^{(t)}$\;
\Return $(\hat{y}, \hat{c}, \mathcal{E}_t)$\;
\end{algorithm}

